Understanding the Quality of Container Security Vulnerability Detection Tools

Virtualization enables information and communications technology industry to better manage computing resources. In this regard, improvements in virtualization approaches together with the need for consistent runtime environment, lower overhead and smaller package size has led to the growing adoption of containers. This is a technology, which packages an application, its dependencies and Operating System (OS) to run as an isolated unit. However, the pressing concern with the use of containers is its susceptibility to security attacks. Consequently, a number of container scanning tools are available for detecting container security vulnerabilities. Therefore, in this study, we investigate the quality of existing container scanning tools by proposing two metrics that reflects coverage and accuracy. We analyze 59 popular public container images for Java applications hosted on DockerHub using different container scanning tools (such as Clair, Anchore, and Microscanner). Our findings show that existing container scanning approach does not detect application package vulnerabilities. Furthermore, existing tools do not have high accuracy, since 34% vulnerabilities are being missed by the best performing tool. Finally, we also demonstrate quality of Docker images for Java applications hosted on DockerHub by assessing complete vulnerability landscape i.e., number of vulnerabilities detected in images.

==> table/osissues.tex <==
\pgfplotstabletypeset[
  col sep=comma,
  columns/name/.style={
  		string type,
  		column name=\textbf{OS}, 
		column type={l}
  },
  columns/osfreq/.style={
  	string type,
	column name=\textbf{Image using OS}, 
	column type={r}
	},	
  columns/bugfreq/.style={	
    	string type,
	column name=\textbf{\#Bug},
    	column type={r}
  },
    columns/pacfreq/.style={	
    	string type,
	column name=\textbf{\#Affected Packages},
    	column type={r}
  },
 every head row/.style={
  					before row={		
								\toprule
							  },
					after row=\bottomrule				     },
  every last row/.style={after row=\bottomrule},
  ]{./table/data/bubble.csv}



==> table/ospackagetable.tex <==
\pgfplotstabletypeset[
  col sep=comma,
  columns/os/.style={
  		string type,
  		column name=\textbf{OS}, 
		column type={l}
  },
  columns/package/.style={
  	string type,
	column name=\textbf{Package}, 
	column type={c}
	},	
  columns/vulnerability/.style={	
    	string type,
	column name=\textbf{Vulnerability},
    	column type={l}
  },
 every head row/.style={
  					before row={		
								\hline
							  },
					after row=\hline
				     },
  every last row/.style={after row=\hline},
  ]{./table/data/mostvulostable.csv}



==> table/vultable.tex <==

\pgfplotstabletypeset[
  col sep=comma,
  columns/name/.style={
  		string type,
  		column name=\textbf{Name}, 
		column type={l}
  },
  columns/totalvulclass/.style={
  	string type,
	column name=\textbf{Vulnerable Class}, 
	postproc cell content/.code={%
        		\pgfplotsutilstrreplace{_}{\_}{##1}%
        		\pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
    	},
	column type={c}
	},	
  columns/bugtype/.style={	
    	string type,
	column name=\textbf{Most Prevalent Bug Type},
    	postproc cell content/.code={%
        		\pgfplotsutilstrreplace{_}{\_}{##1}%
        		\pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
    	},
    	column type={l}
  },
  columns/vulconstructs/.style={
  		string type,
  		column name=\textbf{Vulnerable constructs}, 
		column type={c}
  },
  every head row/.style={
  					before row={		
								\rowcolor[gray]{0.9}
							  },
					%after row=\hline
				     },
  %every last row/.style={after row=\hline},
  ]{./table/data/vultable.csv}




==> table/vultypetable.tex <==
\pgfplotstabletypeset[
  col sep=comma,
  columns/Vultype/.style={
  		string type,
  		column name=\textbf{Vulnerability Type}, 
		column type={l}
  },
  columns/num/.style={
  	string type,
	column name=\textbf{\# Detected Vulnerabilities}, 
	column type={c}
	},	
 every head row/.style={
  					before row={		
								\hline
							  },
					after row=\hline
				     },
  every last row/.style={after row=\hline},
  ]{./table/data/vultype.csv}


